MEMOREPAIR: Barrier-First Cascade Repair in Agentic Memory

Agentic memory evolves across tasks into durable derived artifacts: summaries, cached outputs, embeddings, learned skills, and executable tool procedures. When a source artifact is deleted, corrected, or invalidated by tool or API migration, descendants derived from that source can remain visible and steer future actions with stale support. We formalize this failure mode as the cascade update problem, where repair targets the visible derived state of the memory store. We present MemoRepair, a barrier-first cascade-repair contract for agentic memory. A repair event induces a controlled transition from invalidated descendant state to validated successor state: affected descendants are withdrawn before repair, successors are constructed from retained support and staged repaired predecessors under the current interface, and republication is restricted to validated predecessor-closed successors. This contract induces a scalarized repair-selection problem for a fixed repair-cost tradeoff. We show that the induced publication problem reduces to maximum-weight predecessor closure and can be solved exactly by a single s-t min-cut. Experiments on ToolBench and MemoryArena show that, with complete influence provenance, MemoRepair reduces invalidated-memory exposure from 69.8-94.3% under systems without cascade repair to 0%. Compared with exhaustive Repair all, it recovers 91.1-94.3% of validated successors while reducing normalized repair-operator cost from 1.00 to 0.57-0.76.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}[leftmargin=*]

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction outline the main claims. Details are provided in the following sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses limitations in Section~\ref{sec:conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: The main theoretical result is stated in
Theorem~\ref{thm:cost-aware-repair}; the full min-cut proof is in
Appendix~\ref{app:proof-cost-aware-repair}, with scope and replica
assumptions in Appendix~\ref{app:complexity-guarantees}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section~\ref{sec:experiment} and
    Appendix~\ref{app:reproducibility} describe the experimental setup.
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The implementation code is included in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: Section~\ref{sec:experiment} gives the experimental
setup, with dataset statistics in Appendix~\ref{app:dataset-stats},
hyperparameters in Appendix~\ref{app:hyperparameters}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: The main results are reported as means over three
seeds, and Appendix~\ref{app:std-tables} reports the corresponding per-cell
standard deviations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: Appendix~\ref{app:hardware-software} reports the
hardware and software setup.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research uses public benchmarks and released model/checkpoint assets, preserves submission anonymity, and does not involve human-subject data collection or procedures that deviate from the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses broader impacts in Appendix~\ref{sec:impact}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release a new high-risk pretrained model, scraped dataset, image generator, or other dual-use asset requiring controlled-release safeguards. Experiments use public benchmarks and released checkpoints.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Existing benchmarks, datasets, model checkpoints, and baseline systems are cited in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code used to conduct our experiments is included in the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or human-subject experiments. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve human-subject participants.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLM is used for manuscript review, wording refinement, and clarity checks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> problem_and_algorithm.tex <==
% ================================================================
\section{Problem Setup}
\label{sec:problem}

We formalize the \emph{cascade update problem} as safe, budgeted repair in agentic memory systems. Persistent memory stores durable artifacts---records, summaries, cached outputs, learned skills, and
executable tool procedures---linked by provenance edges that record derivation. When a source artifact is deleted, corrected, or migrated, updating that source alone is insufficient: descendant artifacts can
remain visible and continue to influence system behavior. A repair
event must therefore transform the visible state induced by the
affected descendants. We use the standard Lagrangian form of a budgeted
selection problem, in which a fixed tradeoff parameter $\lambda \geq 0$
traces the repair--budget frontier.

% ----------------------------------------------------------------
\subsection{Core objects and notation}
\label{subsec:notation}

\paragraph{Memory provenance graph.}
The system maintains derivation relationships among durable artifacts
as a directed graph
\[
\G = (V,\, E^{\mathrm{inf}},\, E^{\mathrm{sem}}),
\]
where:
\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item $V$ is the set of durable memory artifacts (nodes). Each
  artifact $x \in V$ has a kind tag
  $\mathrm{kind}(x) \in \{\mathsf{record}, \mathsf{cache},
  \mathsf{summary}, \mathsf{skill}\}$ and, for skills, an architecture
  tag $\mathrm{arch}(x) \in \{\mathsf{neural}, \mathsf{prompt},
  \mathsf{chain}\}$.
  \item $E^{\mathrm{inf}} \subseteq V \times V$: \emph{influence edges}. $(u,v) \in E^{\mathrm{inf}}$ means $v$ was causally derived from $u$. Influence edges determine repair scope.
  \item $E^{\mathrm{sem}} \subseteq V \times V$: \emph{semantic edges}, supporting retrieval but \emph{not} determining repair scope.
\end{itemize}

\paragraph{Repair event.}
A repair event $e = (F, \tau, \Delta)$ consists of:
\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item $F \subseteq V$: the \emph{invalidated root set}.
  \item $\tau \in \{\mathsf{delete}, \mathsf{correct},
  \mathsf{migrate}\}$: the \emph{event type}.
  \item $\Delta$: optional \emph{replacement information}. Empty for
  deletion; for correction, $\Delta$ contains the replacement root
  $x_\Delta \in V$; for migration, $\Delta$ is a contract delta.
\end{itemize}
$\tau$ describes the operation on \emph{root} artifacts in $F$; it is
distinct from the repair mode $\mu_i$
(Section~\ref{subsec:recovery}), which describes how each
\emph{descendant} $i \in D(F)$ is repaired.

\paragraph{Affected cascade and descendants.}
\[
C(F) = \operatorname{Reach}(F;\, E^{\mathrm{inf}}), \qquad
D(F) = C(F) \setminus F.
\]
Only $E^{\mathrm{inf}}$ determines cascade scope.

\paragraph{Replicas and visibility.}
$\mathcal{M}$: set of all replicas; $\mathcal{R}_e \subseteq
\mathcal{M}$: reachable replicas during event $e$;
$\mathsf{Vis}_r(x) \in \{0,1\}$: whether artifact $x$ is servable on
replica $r$.

\paragraph{Interface contract.}
$\kappa$: contract before repair; $\kappa_e$: contract after $e$. For
deletion and correction, $\kappa_e = \kappa$. For migration,
$\kappa_e$ is obtained by applying $\Delta$ to $\kappa$.

\paragraph{Retained support.}
\[
\mathsf{Ret}(e) = \begin{cases}
V \setminus F & \tau = \mathsf{delete}, \\
(V \setminus F) \cup \{x_\Delta\} & \tau = \mathsf{correct}, \\
V \setminus F & \tau = \mathsf{migrate}.
\end{cases}
\]
For migration, only the contract updates; no root artifact is added.

\paragraph{Validation oracle.}
$\Validate_i(x') \in \{0,1\}$ denotes the mode-appropriate validation
oracle for artifact $i$'s candidate successor $x'$. For
$\mu_i = \mathsf{exact}$, it checks replay consistency against
$\mathsf{Ret}(e)$. For $\mu_i = \mathsf{regen}$, it checks schema
validity, held-out task regression, privacy and safety probes,
and---for $\mathrm{arch}(i)=\mathsf{chain}$---sandbox execution under
$\kappa_e$. For $\mu_i = \mathsf{unlearn}$, it applies the
$\mathsf{regen}$ checks plus forget-set probes on $\mathsf{For}_i(e)$
to verify suppression and retained-utility evaluation on
$\mathsf{Ref}_i(e)$.

\paragraph{Neural skill support and invalidated support.}
For each $i \in V$ with $\mathrm{arch}(i) = \mathsf{neural}$, let
$D_i$ denote the \emph{training support set} of skill $i$: the
multiset of labeled examples $(x_j, y_j)$ used to produce the current
adapter $\Delta\theta_i$. The function
$\mathrm{provenance}(x_j, y_j) \subseteq V$ maps each support example
to the set of root artifacts in $\G$ that induced it.

For each $i \in D(F)$ with $\mathrm{arch}(i) = \mathsf{neural}$ and
repair event $e = (F, \tau, \Delta)$, define:
\begin{align*}
\mathsf{For}_i(e) &= \bigl\{(x_j,y_j)\in D_i :
  \mathrm{provenance}(x_j,y_j)\cap F \neq \varnothing\bigr\}, \\
\mathsf{New}_i(e) &= \begin{cases}
  \mathrm{Materialize}(x_\Delta,\, i)
  & \tau=\mathsf{correct}, \\
  \varnothing & \text{otherwise,}
\end{cases}\\
\mathsf{Ref}_i(e) &=
  \bigl(D_i \setminus \mathsf{For}_i(e)\bigr) \cup \mathsf{New}_i(e).
\end{align*}
$\mathsf{For}_i(e)$ is the \emph{forget set}: support examples whose
provenance intersects the invalidated roots $F$.
$\mathsf{New}_i(e)$ is the \emph{replacement support}: newly
materialized training examples derived from the correction replacement
$x_\Delta$ at repair time; these are not required to be in $D_i$.
$\mathsf{Ref}_i(e)$ is the \emph{reference set} passed to the
unlearning operator: retained examples from $D_i$ augmented with any
freshly materialized replacement support. The function
$\mathrm{Materialize}(x_\Delta, i)$ generates new support examples for
skill $i$ from $x_\Delta$ using the same derivation procedure that
produced $D_i$; for deletion and migration,
$\mathsf{Ref}_i(e) = D_i \setminus \mathsf{For}_i(e)$.

\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ll}
\toprule
\textbf{Symbol} & \textbf{Meaning} \\
\midrule
$\G = (V, E^{\mathrm{inf}}, E^{\mathrm{sem}})$ & memory provenance graph \\
$V$ & durable memory artifacts (nodes) \\
$E^{\mathrm{inf}}$ & influence edges (determine repair scope) \\
$E^{\mathrm{sem}}$ & semantic edges (retrieval; not repair scope) \\
$\mathrm{kind}(x)$ & artifact kind: record, cache, summary, or skill \\
$\mathrm{arch}(x)$ & skill architecture: neural, prompt, or chain \\
$e = (F, \tau, \Delta)$ & repair event: root set, type, replacement info \\
$F \subseteq V$ & invalidated root set \\
$\tau$ & event type: delete, correct, or migrate (root op.) \\
$\Delta$ & replacement info ($x_\Delta \in V$ for correct) \\
$x_\Delta \in V$ & replacement root artifact contained in $\Delta$ \\
$C(F)$ & affected cascade $= \operatorname{Reach}(F; E^{\mathrm{inf}})$ \\
$D(F)$ & affected descendants $= C(F) \setminus F$ \\
$\mathcal{M}$ & set of all replicas \\
$\mathcal{R}_e \subseteq \mathcal{M}$ & replicas reachable during event $e$ \\
$\mathsf{Vis}_r(x) \in \{0,1\}$ & whether $x$ is servable on replica $r$ \\
$\kappa$ & interface contract before repair \\
$\kappa_e$ & interface contract after event $e$ \\
$\mathsf{Ret}(e) \subseteq V$ & retained support (store level) \\
$D_i$ & training support set of neural skill $i$ \\
$\mathrm{provenance}(x_j,y_j) \subseteq V$ & root artifacts in $\G$ that induced example $(x_j,y_j)$ \\
$\mathsf{For}_i(e) \subseteq D_i$ & forget set: examples with provenance intersecting $F$ \\
$\mathsf{New}_i(e)$ & replacement support materialized from $x_\Delta$ (correction only) \\
$\mathsf{Ref}_i(e)$ & reference set $= (D_i\setminus\mathsf{For}_i(e))\cup\mathsf{New}_i(e)$ \\
$\mathrm{Materialize}(x_\Delta,i)$ & generates new support examples for skill $i$ from $x_\Delta$ \\
$\Validate_i(x') \in \{0,1\}$ & mode-appropriate validation oracle for candidate $x'$ of $i$ \\
$\mu_i$ & repair mode: remove, exact, regen, or unlearn \\
$D^+(F)$ & repairable descendants $= \{i \in D(F) : \mu_i \neq \mathsf{remove}\}$ \\
$Q_e = \{q_i\}_{i \in D^+(F)}$ & full candidate family (may include $v_i=0$) \\
$\widehat{Q}_e \subseteq Q_e$ & executable candidate family $= \{q_i \in Q_e : v_i = 1\}$ \\
$q_i = (\mu_i, \pi_i, P_i, v_i, w_i, c_i)$ & candidate repair tuple for $i \in D^+(F)$ \\
$\pi_i$ & recovery operator for descendant $i$ \\
$\pi_i^{\mathsf{unlearn}}$ & unlearning operator for neural descendant $i$ \\
$P_i \subseteq D^+(F)$ & affected predecessors required before $i$ can be repaired \\
$v_i \in \{0,1\}$ & whether executable candidate repair exists for $i$ \\
$w_i \geq 0$ & repair value of restoring $i$ \\
$c_i \geq 0$ & repair cost of restoring $i$ \\
$E^{\mathrm{req}}$ & induced repair dependency graph over $D^+(F)$ \\
$x_i \in \{0,1\}$ & decision variable: repair of $i$ selected? \\
$\lambda \geq 0$ & cost--benefit tradeoff parameter \\
$p_i = w_i - \lambda c_i$ & net profit of repairing descendant $i$ \\
$\rho = (B_\rho, Q_\rho, S_\rho, R_\rho)$ & repair plan \\
$B_\rho \subseteq V$ & hidden set (withdrawn from service) \\
$Q_\rho = \{q_i\}_{i \in D^+(F)}$ & candidate repair family associated with plan $\rho$ \\
$S_\rho \subseteq D^+(F)$ & selected descendants for repair in current epoch \\
$R_\rho \subseteq S_\rho \times V$ & republished successor pairs $(i, x_i')$ \\
\bottomrule
\end{tabular}
\caption{Notation used in the problem formulation.}
\label{tab:notation}
\end{table}

% ----------------------------------------------------------------
\subsection{Artifact repair modes}
\label{subsec:recovery}

Each affected descendant $i \in D(F)$ is assigned a repair mode
$\mu_i \in \{\mathsf{remove},\, \mathsf{exact},\,
\mathsf{regen},\, \mathsf{unlearn}\}$:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item \textbf{Permanent removal} ($\mu_i = \mathsf{remove}$): no
  meaningful successor under $\mathsf{Ret}(e)$ and $\kappa_e$; removed
  immediately and does not enter the optimization.
  \item \textbf{Exact recomputation} ($\mu_i = \mathsf{exact}$):
  deterministic function of parents; rebuilt exactly from
  $\mathsf{Ret}(e)$.
  \item \textbf{Retained-support regeneration} ($\mu_i = \mathsf{regen}$):
  non-neural compressive artifact (summary, prompt skill, or chain
  procedure); regenerated from retained valid sources under $\kappa_e$;
  exact causal equivalence is not claimed.
  \item \textbf{Best-effort unlearning} ($\mu_i = \mathsf{unlearn}$):
  parametric neural skill with entangled adapter weights; apply
  $\pi_i^{\mathsf{unlearn}}$ with forget set $\mathsf{For}_i(e)$ and
  reference set $\mathsf{Ref}_i(e)$ under $\kappa_e$; republished only
  if $\Validate_i(x_i') = 1$; exact parameter-level erasure is not
  claimed. In our default instantiation for LoRA-trained skills,
  $\pi_i^{\mathsf{unlearn}}$ is LUNE~\citep{lune2025} for single-epoch
  repairs and OOO~\citep{ooo2024} when the same skill undergoes multiple
  sequential repair epochs; both operators require $\mathsf{For}_i(e)$
  and $\mathsf{Ref}_i(e)$ and are executable only when
  $\mathsf{Ref}_i(e) \neq \varnothing$.
\end{itemize}

Note: $\tau = \mathsf{delete}$ deletes a \emph{root} in $F$; $\mu_i =
\mathsf{remove}$ permanently removes a \emph{descendant} in $D(F)$.

The \emph{repairable descendants} are $D^+(F) = \{i \in D(F) : \mu_i
\neq \mathsf{remove}\}$.

\paragraph{Candidate repair tuple.}
For each $i \in D^+(F)$, candidate generation produces
$q_i = (\mu_i, \pi_i, P_i, v_i, w_i, c_i)$, where:
\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item $\mu_i \in \{\mathsf{exact}, \mathsf{regen}, \mathsf{unlearn}\}$
  (remove-mode descendants do not enter $D^+(F)$);
  \item $\pi_i$: recovery operator for mode $\mu_i$ and
  $\mathrm{kind}(i)$; for $\mu_i = \mathsf{unlearn}$,
  $\pi_i = \pi_i^{\mathsf{unlearn}}$;
  \item $P_i \subseteq D^+(F)$: affected predecessors whose candidate
  successors must be available before $i$ can be republished;
  \item $v_i \in \{0,1\}$: $1$ iff $\pi_i$ is executable using the
  resources required by its repair mode, $\kappa_e$, and the staged or
  republished successors of all $j \in P_i$; for $\mu_i =
  \mathsf{unlearn}$, additionally requires $\mathsf{For}_i(e)$ to be
  materializable from $\G$ and $\mathsf{Ref}_i(e) \neq \varnothing$.
  After $E^{\mathrm{req}}$ is constructed, any descendant $i$ that
  lies in a non-trivial SCC of $E^{\mathrm{req}}$ is assigned $v_i = 0$
  and quarantined, because no execution order can satisfy mutual
  predecessor requirements within a cycle;
  \item $w_i \geq 0$, $c_i \geq 0$: repair value and cost.
\end{itemize}

\paragraph{Induced repair dependency graph.}
$E^{\mathrm{req}} = \{(j,i) \in D^+(F) \times D^+(F) : j \in P_i\}$.
Edge $(j,i)$: the staged or republished successor of $j$ must be
available before $\pi_i$ can execute.

The \emph{full candidate family} is $Q_e = \{q_i\}_{i \in D^+(F)}$,
which may include candidates with $v_i = 0$. After constructing
$E^{\mathrm{req}}$, every node lying in a non-trivial SCC is assigned
$v_i = 0$ and excluded from the \emph{executable candidate family}:
\[
\widehat{Q}_e = \{q_i \in Q_e : v_i = 1\}.
\]
Hence $E^{\mathrm{req}}[\widehat{Q}_e]$ is a DAG.

% ----------------------------------------------------------------
\subsection{Repair events and feasible repair plans}
\label{subsec:repair-feasible}

\begin{definition}[Repair event]
\label{def:repair-event}
A \emph{repair event} is $e = (F, \tau, \Delta)$ where $F \subseteq V$,
$\tau \in \{\mathsf{delete}, \mathsf{correct}, \mathsf{migrate}\}$,
and $\Delta$ is optional replacement information.
\end{definition}

\paragraph{Event semantics.}
For $\tau = \mathsf{delete}$: roots removed, $\mathsf{Ret}(e) = V
\setminus F$. For $\tau = \mathsf{correct}$: $x_\Delta$ installed,
$\mathsf{Ret}(e) = (V \setminus F) \cup \{x_\Delta\}$. For $\tau =
\mathsf{migrate}$: contract updates to $\kappa_e$, $\mathsf{Ret}(e) =
V \setminus F$; here $V \setminus F$ excludes obsolete pre-migration
artifact versions, while the post-event interface $\kappa_e$ supplies
the migrated contract or handle used by replay and validation. The
optimization applies only to $D^+(F)$.

\begin{definition}[Feasible repair plan]
\label{def:feasible}
A \emph{repair plan} $\rho = (B_\rho, Q_\rho, S_\rho, R_\rho)$ is
\emph{feasible} if all five conditions hold.
\begin{enumerate}[leftmargin=*,label=(\roman*),itemsep=2pt]
  \item \textbf{Coverage.} $C(F) \subseteq B_\rho$.

  \item \textbf{Withdrawal barrier.}
  For every $r \in \mathcal{R}_e$ and $i \in B_\rho$,
  $\mathsf{Vis}_r(i) = 0$ until: (a) $i$ is permanently removed
  ($\mu_i = \mathsf{remove}$ for $i \in D(F)$, or $i \in F$ for any
  $\tau$---all roots are permanently superseded regardless of event
  type); (b) a validated successor $x_i'$ is published and
  $(i, x_i') \in R_\rho$; or (c) $i$ is quarantined after failed
  repair, remaining in $B_\rho$ with $\mathsf{Vis}_r(i) = 0$.
  Any replica in $\mathcal{R}_e$ that does not acknowledge withdrawal
  of $B_\rho$ within $T_{\mathrm{ack}}$ is fenced: it is removed from
  $\mathcal{R}_e$ and blocked from serving until it reconnects and
  merges $B_\rho$.

  \item \textbf{Candidate executability.}
  For every $q_i \in Q_\rho$ with $v_i = 1$, $\pi_i$ is executable
  using the resources required by its repair mode, $\kappa_e$, and the
  staged or republished successors of all $j \in P_i$. For $\mu_i \in
  \{\mathsf{exact}, \mathsf{regen}\}$, these resources are derived from
  $\mathsf{Ret}(e)$. For $\mu_i = \mathsf{unlearn}$, they additionally
  include the current adapter $\Delta\theta_i$ together with
  $\mathsf{For}_i(e)$ and $\mathsf{Ref}_i(e)$.

  \item \textbf{Selection closure.}
  If $i \in S_\rho$ and $j \in P_i$, then $j \in S_\rho$.

  \item \textbf{Validated republication.}
  If $(i, x_i') \in R_\rho$: $i \in S_\rho$, $v_i = 1$, and either
  (a) $\mu_i = \mathsf{exact}$: $x_i'$ recomputed from
  $\mathsf{Ret}(e)$, $\Validate_i(x_i') = 1$; or
  (b) $\mu_i = \mathsf{regen}$: $x_i'$ produced from $\mathsf{Ret}(e)$
  and $\kappa_e$, $\Validate_i(x_i') = 1$; or
  (c) $\mu_i = \mathsf{unlearn}$: $x_i'$ produced by applying
  $\pi_i^{\mathsf{unlearn}}$ with forget set $\mathsf{For}_i(e)$ and
  reference set $\mathsf{Ref}_i(e)$ under $\kappa_e$,
  $\Validate_i(x_i') = 1$.
  Failure under any mode quarantines $i$ per condition~(ii).
\end{enumerate}
\end{definition}

% ----------------------------------------------------------------
\subsection{Budgeted repair selection}
\label{subsec:budgeted}

For each $i \in D^+(F)$, let $x_i \in \{0,1\}$ and define:
\[
\mathrm{Repair}(x) = \textstyle\sum_{i \in D^+(F)} w_i x_i, \quad
\mathrm{Budget}(x) = \textstyle\sum_{i \in D^+(F)} c_i x_i.
\]
\begin{align}
x_i &\leq v_i, && \forall i \in D^+(F), \label{eq:avail}\\
x_i &\leq x_j, && \forall j \in P_i,\;\forall i \in D^+(F),
\label{eq:closure}\\
x_i &\in \{0,1\}, && \forall i \in D^+(F). \label{eq:binary}
\end{align}
Let $\lambda \geq 0$ be the fixed tradeoff parameter. The
\emph{budgeted repair-selection problem} is:
\[
\max_{x}\;\mathrm{Repair}(x)-\lambda\cdot\mathrm{Budget}(x)
\quad\text{s.t.\ \eqref{eq:avail}--\eqref{eq:binary}.}
\]
Constraint~\eqref{eq:avail} uses $v_i$ from the full candidate family
$Q_e$; candidates with $v_i = 0$ (including all cyclic descendants)
are excluded from the feasible region. In the implementation, the
executable family $\widehat{Q}_e$ is passed directly to
\textsc{MinCutSelect}, which is equivalent because all $v_i = 0$
candidates are forced out by the $M$-penalty construction in the proof
of Theorem~\ref{thm:closure}. Since $E^{\mathrm{req}}[\widehat{Q}_e]$
is a DAG, topological execution order over $S^\star$ is well-defined.

\paragraph{Interpretation.}
Selects candidate successors to produce and republish; not an
optimization over causal erasure. For $\mu_i = \mathsf{exact}$: exact
recomputation. For compressive artifacts: $w_i$ scores the validated
retained-support successor.

\begin{theorem}[Fixed-$\lambda$ budgeted repair selection]
\label{thm:closure}
Fix $e$, $Q_e$ over $D^+(F)$, and $\lambda \geq 0$. The budgeted
repair-selection problem over $E^{\mathrm{req}}$ reduces to a
maximum-weight closure problem and can be solved to optimality by a
single $s$-$t$ min-cut~\citep{picard1976closure}.
\end{theorem}

\begin{proof}[Proof sketch]
Let $p_i = w_i - \lambda c_i$ and $W^+ = \sum_{i:\,p_i>0} p_i$.
Construct a flow network with source $s$ and sink $t$. For each $i$:
add $s\to i$ (cap $p_i$) if $p_i>0$; add $i\to t$ (cap $-p_i$) if
$p_i<0$; add $i\to t$ (cap $M>W^+$) if $v_i=0$. The $v_i=0$ rule is
cumulative: if $v_i=0$ and $p_i>0$, both $s\to i$ and $i\to t$ (cap
$M$) are added; the $M$-edge dominates in any minimum cut. For each
$(j,i)\in E^{\mathrm{req}}$: add $i\to j$ (cap $M$).

The empty set $U=\varnothing$ induces a cut of capacity $W^+$. Any
cut in which $i\in U$ but $j\notin U$ for some $j\in P_i$ cuts the
dependency edge $i\to j$ at cost $M>W^+$. Any cut containing $i$
with $v_i=0$ cuts an exclusion edge at cost $M>W^+$. Since both
penalties exceed $W^+$, no minimum cut pays either. Every minimum cut
therefore induces a closed, availability-respecting $U\subseteq
D^+(F)$, with cut capacity $W^+-\sum_{i\in U}p_i$. Minimizing cut
capacity maximizes $\sum_{i\in U}p_i = \mathrm{Repair}(x)-\lambda
\cdot\mathrm{Budget}(x)$.
\end{proof}

% ----------------------------------------------------------------
\subsection{Lineage and affected cascades}
\label{subsec:lineage}

The system maintains raw provenance as an execution--artifact graph
$\mathcal{G}_{\mathrm{prov}} = (\mathcal{X}\cup\mathcal{A},
E_{\mathrm{prov}})$, where $\mathcal{X}$ (executions) and
$\mathcal{A}$ (artifact records) are local to this subsection. Because
memory updates can be iterative, $\mathcal{G}_{\mathrm{prov}}$ may
contain cycles. The system condenses strongly connected components and
projects onto $\G = (V,E^{\mathrm{inf}},E^{\mathrm{sem}})$.
Reachability is preserved under condensation, so $C(F)$ is computable
on $\G$.

% ----------------------------------------------------------------
\subsection{Scope}
\label{subsec:scope}

All guarantees are store-level under complete provenance: stale
artifacts are withdrawn on all replicas in $\mathcal{R}_e$ and
republished successors must pass $\Validate_i$. For $\mu_i \in
\{\mathsf{exact}, \mathsf{regen}\}$, successors are built from
retained support $\mathsf{Ret}(e)$ under $\kappa_e$. For $\mu_i =
\mathsf{unlearn}$, successors are produced by applying the unlearning
operator to the current neural artifact using forget and reference
support derived from provenance under $\kappa_e$; exact
parameter-level erasure is not claimed unless the operator provides an
explicit guarantee. Flat retrieval-only stores that do not maintain
$E^{\mathrm{inf}}$ cannot identify $C(F)$ and are outside the scope of
these guarantees.

% ================================================================
\section{\textsc{BarrierRepair}}
\label{sec:framework}

\subsection{Overview}
\label{subsec:overview}

\textsc{BarrierRepair} operates in four stages. It first localizes the
affected cascade $C(F)$, then enforces a withdrawal barrier on
reachable replicas $\mathcal{R}_e$, next generates artifact-specific
repair candidates and selects a dependency-closed repair set $S^\star$
by min-cut on the executable family $\widehat{Q}_e$, and finally
executes and validates selected repairs node by node in topological
order and commits all validated successors in a single batch visibility
operation.

% ----------------------------------------------------------------
\subsection{Withdrawal barrier}
\label{subsec:withdrawal}

Let $T_{\mathrm{ack}} > 0$ be the acknowledgement timeout (wall-clock
seconds). The hidden set is initialized to $B_\rho \leftarrow C(F)$
and propagated to $\mathcal{R}_e$; the barrier waits up to
$T_{\mathrm{ack}}$ for acknowledgement from every replica in
$\mathcal{R}_e$. Any replica that does not acknowledge within
$T_{\mathrm{ack}}$ is fenced: it is removed from $\mathcal{R}_e$ and
blocked from serving until it reconnects and merges $B_\rho$. Repair
begins only after all remaining replicas in $\mathcal{R}_e$ have
acknowledged. A remove-wins CRDT ensures no merge makes a withdrawn
artifact visible again. Fenced replicas merge $B_\rho$ on reconnection
before rejoining $\mathcal{R}_e$. Requests touching hidden artifacts
fall back to the nearest non-hidden ancestor; fallback deactivates as
validated successors are published.

% ----------------------------------------------------------------
\subsection{Root update, candidate generation, and repair selection}
\label{subsec:optstep}

Apply root update per event semantics
(Section~\ref{subsec:repair-feasible}). For each $i\in D(F)$,
\textsc{CandidateRepair} assigns a repair mode $\mu_i \in
\{\mathsf{remove},\mathsf{exact},\mathsf{regen},\mathsf{unlearn}\}$.
Remove-mode descendants are deleted permanently. The repairable set is
$D^+(F) = \{i \in D(F) : \mu_i \neq \mathsf{remove}\}$.

Candidate generation produces the full family $Q_e = \{q_i\}_{i \in
D^+(F)}$ with dependency graph:
\[
E^{\mathrm{req}} = \{(j,i)\in D^+(F)^2 : j\in P_i\}.
\]
After $E^{\mathrm{req}}$ is constructed, every node in a non-trivial
SCC is assigned $v_i = 0$ and quarantined. All remaining candidates
with $v_i = 0$ (non-executable for any reason) are retained in $Q_e$
for audit but excluded from the executable family:
\[
\widehat{Q}_e = \{q_i \in Q_e : v_i = 1\}.
\]
$E^{\mathrm{req}}[\widehat{Q}_e]$ is a DAG by construction.
Solve Theorem~\ref{thm:closure} on $\widehat{Q}_e$ to obtain
$S^\star \subseteq D^+(F)$.

\paragraph{Repair execution.}
Topologically order $S^\star$ by $E^{\mathrm{req}}[S^\star]$. For each
$i \in S^\star$ in this order, all $j \in P_i$ have already been
staged, so $\{Z[j]\}_{j \in P_i}$ is fully available, satisfying the
executability condition $v_i = 1$ exactly as stated in
Section~\ref{subsec:recovery}. Apply the mode-appropriate operator:
for $\mathsf{exact}$: deterministic recompute from $\mathsf{Ret}(e)$;
for $\mathsf{regen}$: regenerate from $\mathsf{Ret}(e)$ under
$\kappa_e$; for $\mathsf{unlearn}$: apply
$\pi_i^{\mathsf{unlearn}}$ to the current adapter $\Delta\theta_i$
using forget set $\mathsf{For}_i(e)$ and reference set
$\mathsf{Ref}_i(e)$ under $\kappa_e$; the base model
$\theta_{\mathrm{base}}$ is not modified.

\paragraph{Validation and batch publication.}
After all nodes in $S^\star$ are staged, each node $i \in S^\star$ is
tested individually by $\Validate_i(Z[i])$. If every node passes, all
successors $\{Z[i]\}_{i \in S^\star}$ are committed by a single batch
visibility operation $\mathrm{PublishBatch}(\{(i,Z[i]) : i \in
S^\star\})$; $(i, Z[i])$ is then recorded in $R_\rho$ and linked by
$\mathsf{replaces}(i,Z[i])$ in $\G$, and fallback deactivates for each
published node. If any node $i \in S^\star$ fails validation, it is
quarantined ($v_i \leftarrow 0$), its staged output is discarded,
$\widehat{Q}_e$ is pruned of $i$ and any node whose closure now
requires $i$, and the selection is re-solved on the residual
$\widehat{Q}_e$. The final published set is optimal for the residual
executable family at the time of publication, preserving the
optimality guarantee of Theorem~\ref{thm:closure} for that family.

\paragraph{Concurrent repair.}
Concurrent repair requests are ordered by Lamport
timestamp~\citep{lamport1978time}. Overlapping epochs: the earlier
completes first. Deletion events take precedence over correction and
migration for the same root. Repairs on disjoint subgraphs of $\G$
proceed independently.

% ----------------------------------------------------------------
\subsection{Algorithm}
\label{subsec:algorithm}

\textsc{MinCutSelect}$(\widehat{Q}_e,\lambda)$ constructs the flow
network from Theorem~\ref{thm:closure} on the executable family
$\widehat{Q}_e$ and returns the source-side min-cut node set $S^\star$.

\begin{algorithm}[t]
\caption{\textsc{BarrierRepair}$(\G,\,e,\,T_{\mathrm{ack}},\,\lambda)$}
\label{alg:barrier}
\begin{algorithmic}[1]
\STATE Parse $e=(F,\tau,\Delta)$
  \COMMENT{$\tau\in\{\mathsf{delete},\mathsf{correct},\mathsf{migrate}\}$}
\STATE $C \leftarrow \Reach(F;\,E^{\mathrm{inf}})$
  \COMMENT{affected cascade $C(F)$}
\STATE $B_\rho \leftarrow C$; broadcast $B_\rho$ to $\mathcal{R}_e$; activate fallback
\STATE Wait up to $T_{\mathrm{ack}}$ for acknowledgements from $\mathcal{R}_e$
\STATE Fence non-acknowledging replicas; remove from $\mathcal{R}_e$
  \COMMENT{barrier complete; repair begins}
\STATE $\G \leftarrow \mathrm{ApplyRootUpdate}(\G,e)$
  \COMMENT{update $\mathsf{Ret}(e)$, $\kappa_e$;
           materialize $\mathsf{New}_i(e)$ for neural descendants
           if $\tau=\mathsf{correct}$}
\STATE $D \leftarrow C \setminus F$
  \COMMENT{affected descendants $D(F)$}
\STATE $Q_e \leftarrow \emptyset$;\quad $\widehat{Q}_e \leftarrow \emptyset$
\FORALL{$i \in D$}
  \STATE $(\mathrm{status}_i,\,q_i) \leftarrow \mathrm{CandidateRepair}(i,\,e)$
  \IF{$\mathrm{status}_i = \texttt{remove}$}
    \STATE Remove $i$ permanently; record audit event
      \COMMENT{$\mu_i=\mathsf{remove}$: no valid successor}
  \ELSIF{$\mathrm{status}_i = \texttt{repairable}$}
    \STATE $Q_e \leftarrow Q_e \cup \{q_i\}$
      \COMMENT{$v_i=1$ pending SCC check; $\mu_i\in\{\mathsf{exact},\mathsf{regen},\mathsf{unlearn}\}$}
  \ELSE
    \STATE $Q_e \leftarrow Q_e \cup \{q_i\}$;\quad quarantine $i$; record audit event
      \COMMENT{$v_i=0$: non-executable; in $Q_e$ for audit only}
  \ENDIF
\ENDFOR
\STATE Build $E^{\mathrm{req}} = \{(j,i)\in D^+(F)^2 : j\in P_i\}$
\STATE Detect non-trivial SCCs of $E^{\mathrm{req}}$
\FORALL{$i$ in a non-trivial SCC of $E^{\mathrm{req}}$}
  \STATE Set $v_i \leftarrow 0$;\quad quarantine $i$; record audit event
    \COMMENT{cyclic dependency: unsatisfiable predecessor requirements}
\ENDFOR
\STATE $\widehat{Q}_e \leftarrow \{q_i \in Q_e : v_i = 1\}$
  \COMMENT{$E^{\mathrm{req}}[\widehat{Q}_e]$ is a DAG}
\WHILE{$\widehat{Q}_e \neq \emptyset$}
  \STATE $S^\star \leftarrow \mathrm{MinCutSelect}(\widehat{Q}_e,\,\lambda)$
  \IF{$S^\star = \emptyset$}
    \STATE \textbf{break}
  \ENDIF
  \STATE Topologically order $S^\star$ by $E^{\mathrm{req}}[S^\star]$
  \STATE $Z \leftarrow \emptyset$
    \COMMENT{staging area}
  \FORALL{$i \in S^\star$ in topological order}
    \STATE $Z[i] \leftarrow \mathrm{ExecuteRepair}(i,\,\mu_i,\,\pi_i,\,
           \{Z[j]\}_{j \in P_i})$
      \COMMENT{all $j\in P_i$ already staged; $v_i=1$ satisfied exactly}
  \ENDFOR
  \STATE $F_{\mathrm{bad}} \leftarrow \{i \in S^\star : \Validate_i(Z[i]) = 0\}$
    \COMMENT{node-level, mode-appropriate validation}
  \IF{$F_{\mathrm{bad}} = \emptyset$}
    \STATE $\mathrm{PublishBatch}(\{(i,\,Z[i]) : i \in S^\star\})$
      \COMMENT{single batch visibility commit}
    \FORALL{$i \in S^\star$}
      \STATE Record $(i, Z[i])$ in $R_\rho$;
             link $\mathsf{replaces}(i,Z[i])$ in $\G$
      \STATE Deactivate fallback for $i$
    \ENDFOR
    \STATE \textbf{break}
  \ELSE
    \FORALL{$i \in F_{\mathrm{bad}}$}
      \STATE Quarantine $i$; set $v_i \leftarrow 0$
    \ENDFOR
    \STATE $\widehat{Q}_e \leftarrow \mathrm{PruneCandidates}(\widehat{Q}_e,\,F_{\mathrm{bad}})$
      \COMMENT{remove $F_{\mathrm{bad}}$ and dependents; re-solve on residual}
  \ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\paragraph{Complexity.}
Localization: $O(|V|+|E^{\mathrm{inf}}|)$. Broadcast and barrier:
$O(|\mathcal{R}_e|)$. Candidate generation: $O(|D(F)|)$, assuming
$O(1)$ classification per artifact. Building $E^{\mathrm{req}}$ and
SCC detection: $O(|D^+(F)|^2)$. \textsc{MinCutSelect} with
push--relabel: $O(|\widehat{Q}_e|^3) \leq O(|D^+(F)|^3)$.
Topological ordering of $S^\star$:
$O(|S^\star|+|E^{\mathrm{req}}[S^\star]|)$, dominated by the min-cut.
The \textbf{while} loop iterates at most $|\widehat{Q}_e| \leq
|D^+(F)|$ times. Total worst-case:
\[
O\!\left(|D^+(F)|^4\right).
\]
